Parallel Structures in Pre-training Data Yield In-Context Learning

Pre-trained language models (LMs) are capable of in-context learning (ICL): they can adapt to a task with only a few examples given in the prompt without any parameter update. However, it is unclear where this capability comes from as there is a stark distribution shift between pre-training text and ICL prompts. In this work, we study what patterns of the pre-training data contribute to ICL. We find that LMs' ICL ability depends on $\textit{parallel structures}$ in the pre-training data -- pairs of phrases following similar templates in the same context window. Specifically, we detect parallel structures by checking whether training on one phrase improves prediction of the other, and conduct ablation experiments to study their effect on ICL. We show that removing parallel structures in the pre-training data reduces LMs' ICL accuracy by 51% (vs 2% from random ablation). This drop persists even when excluding common patterns such as n-gram repetitions and long-range dependency, showing the diversity and generality of parallel structures. A closer look at the detected parallel structures indicates that they cover diverse linguistic tasks and span long distances in the data.

==> Discussion.tex <==
\section{Discussion}
% \kathy{should be "in addition to" but you already used this phrase and I don't find it that meaningful. I think you could just drop it and start with "our findings..."}
% Our findings on why ICL appears open up new directions for improving the transparency and capability of ICL.
\hh{Maybe combine this with related work. Many questions make more sense in the broader context. e.g., question 1 and 2 also applies to other works studying the effect of pretraining data.}
There are many open questions for future work.
First, how to improve ICL using our findings on parallel structures? One straightforward approach is enhancing parallel structures during pre-training, either by adding more of them to the data or upweighting them when computing the training loss.
\hh{data quality and data selection?}
Second, how much can LMs generalize with ICL? We may be able to characterize the generalization of a LM by measuring the distribution shift between parallel structures in pre-training data and downstream ICL examples that the LM is capable of.
Third, what mechanisms do LMs use to predict parallel structures? Intuitively LMs might use similar mechanisms to predict parallel structures and ICL examples, so understanding mechanisms of predicting parallel structures may also explain mechanisms behind ICL.\hh{But why not directly study ICL then? Is studying PSs easier?}

% Understanding this question can inspire methods to amplify ICL during pre-training \cite{shi2023context} and to predict its failure modes caused by pre-training defects \cite{ladhak-etal-2023-contrastive}.
% In a broader context, improving the transparency of ICL is crucial for tackling AI safety, alignment, and regulatory concerns~\cite{goodman2016european,gabriel2020artificial} and for
% calibrating trust of LMs in high-stake domains 


==> deprecated/Abstract_story2.tex <==
\begin{abstract}
Language models (LMs) pre-trained on natural language are capable of in-context learning (ICL), where they quickly adapt to a task by taking as input the concatenation of a few input-output pairs of the task. We conjecture that ICL emerges due to the ICL examples in pre-training corpus. While this hypothesis seems intuitive, it has not been empirically tested. ICL examples are hard to detect in natural language, so we propose to identify a generalized form of ICL examples, which we define as any two tokens in a document that are sampled from a similar conditional distribution.

We first propose a gradient-based algorithm algorithm to detect ICL examples in natural language. We detect two tokens as an ICL example if fine-tuning an off-the-shelf LM on the conditional probability of the first token for one gradient step increases the conditional probability on the second token.
We find out that ICL examples \textit{(i)} are common in natural language, \textit{(ii)} often span long distances, \textit{(iii)} distribute evenly in natural language, and \textit{(iv)} capture diverse semantic and syntactic patterns. We then study how ICL examples in natural language affect the emergent ICL capability of LMs. Ablation experiments on three model sizes show that \textit{(i)} ICL examples are crucial for ICL to emerge (ablating the parallel structures in the pre-training data reduces the ICL accuracy by 55\%); \textit{(ii)} ICL examples matter more than long-range dependencies in the emergence of ICL; \textit{(iii)} ICL examples that are not n-gram repetitions also help improve ICL.

\end{abstract}


==> deprecated/Abstract_v1_withcomments.tex <==
Language models (LMs) pre-trained on natural language can perform in-context learning (ICL), where they adapt to a task by taking as input the concatenation of a few input-output pairs of the task.
\hh{The first sentence is correct but it should highlight that a) the model condition on examples without parameter updates; b) this ability is unexpected.}
Such ICL prompts\hh{unclear "ICL prompts" = input in the first sentence. please also use "prompt" in the first sent.} are uncommon in natural language, so it remains unclear what properties of natural language yield ICL\hh{The fact that they are uncommon doesn't necessarily mean this is not well understood. There are plenty of work studying this already, what is the gap?}. We hypothesize that ICL emerges because natural language contains diverse \textit{parallel structures}, which we define as any two tokens in a document that are sampled from similar conditional distributions.\hh{Give a simple example} We propose a gradient-based algorithm to detect parallel structures: we detect two tokens as a parallel structure if fine-tuning an off-the-shelf LM on the conditional probability of the first token increases the conditional probability of the second token.\hh{too complex. we can just say learning to predict the earlier token improves prediction of the later token.}

%We first study how parallel structures in the pre-training data affect the emergent ICL capability of pre-trained LMs. Ablation experiments on four model sizes
We show that \textit{(i)} parallel structures are crucial for ICL to emerge\hh{I'd avoid using the word emerge or emergent as it is still debatable whether these abilities are truly emerged. And this is irrelevant to our discussion.} (ablating the parallel structures in the pre-training data reduces the ICL accuracy by \textbf{51\%}); \textit{(ii)} Parallel structures matter more than long-range dependencies; \textit{(iii)} Parallel structures that are not n-gram repetitions also matter.\hh{ii and iii can be removed. There's not enough context - what's the main point to take away from them?}
We then study what parallel structures look like in natural language. We find out that parallel structures \textit{(i)} are common, \textit{(ii)} often span long distances, \textit{(iii)} distribute evenly, and \textit{(iv)} capture diverse semantic and syntactic patterns. \hh{A bit awkward to put them in a list. Can we just use a more natural sentence? Again, what's the takeaway here?}


==> deprecated/Introduction_story2.tex <==
\section{Introduction2}
Language models (LMs) are capable of in-context learning (ICL), where they learn a task by taking as input the concatenation of the input and output of a few task examples. ICL is an emergent capability---LMs pre-trained on natural language are capable of ICL without explicit training on ICL prompts of structured input-output concatenations. \textcolor{red}{We conjecture that ICL emerges actually because natural language already contains significant amount of generalized ICL examples, where we define ICL examples as any two tokens in a document sampled from a similar conditional distribution.}

We first propose a gradient-based algorithm to automatically detect ICL examples in natural language (Figure~\ref{fig1} bottom-left, Section~\ref{sec:detection}). If two tokens have similar conditional distributions, then fine-tuning an off-the-shelf LM on the conditional probability of the first token for one gradient step should increase the conditional probability on the second token. We use this method to score the parallel structure strength between any two tokens in the same document.

We use our algorithm to detect the ICL examples in the OpenWebText corpus and study their properties (Section~\ref{sec:analysis}). We find out that ICL examples in natural language \textit{(i)} are common, \textit{(ii)} often span long distances, \textit{(iii)} distribute evenly, and \textit{(iv)} capture diverse patterns in both semantics and syntax.

Finally, we study how ICL examples in the pre-training corpus relate to the emergent ICL capability (Section~\ref{sec:ablation}). Specifically, we ablate the ICL examples in the pre-training corpus by injecting noise, and use it to continue pre-training an off-the-shelf LM. We compare ablating ICL examples to a baseline where we randomly sample the ablated tokens. We evaluate the ICL capability on ten tasks, and observe that \textbf{ablating ICL examples is $\mathbf{55\%}$ worse (relative) than ablating random tokens} (Figure~\ref{fig1} bottom-right). Because ICL examples are related to long-range dependencies and n-gram repetitions, we conduct additional experiments and show that ICL examples are more crucial than long-range dependencies, and ICL examples that are not repeated n-grams are also crucial.

Our contributions are as follows: \textit{(i)} We propose a statistical algorithm to detect ICL examples in natural language automatically; \textit{(ii)} We study various properties of ICL examples in natural language; \textit{(iii)} \textcolor{blue}{We show empirically with ablation experiments that ICL examples in the pre-training data are crucial for ICL to emerge.}

==> deprecated/Introduction_v1_withcomments.tex <==

Language models (LMs) are capable of in-context learning (ICL), where they adapt to a task by taking as input the concatenation of a few input-output pairs of the task \cite{brown2020language, chowdhery2023palm}.\hh{See comment on first sent in abs}
ICL is an emergent capability---LMs pre-trained on natural language are capable of ICL, even though they are not explicit trained on ICL prompts of input-output concatenations \chen{ just repeats the last sentence;} \cite{wei2022emergent} \hh{this isn't the def of "emergent" and I don't think emergence is relevant. Just highlight the OOD point.}. It is unclear what properties of the pre-training data yield ICL.

\hh{We need to talk about what's missing in prior work to justify that "it is unclear..."}

\chen{I think we need better transition between the last sentence and first sentence here; }
\chen{And i think the motivation is a bit weak, we should talk about why we propose ``parallel structures" in more details; could get some help from Fig 1;}
\hh{Need to state our RQ before the hypothesis.}
While ICL prompts are rare in natural language \cite{brown2020language, xie2021explanation, han-etal-2023-understanding, shin2022effect}, we hypothesize that natural language contains frequent and diverse \textbf{parallel structures}, which we define as two tokens sampled from similar conditional distributions \hh{see comment in figure 1; unclear what's the dist}\mbox{(Figure~\ref{fig1})}. \chen{How about moving this sentence forward, then we define parallel structure}\hh{I agree. first talk about the intuitive story, e.g., while ICL prompts are rare, we observe that NL often contains multiple segments following similar distributions [example]. [definition]. Then say that ICL prompt is a special case of PS.} Our definition of parallel structures is inspired by ICL prompts: input-output tokens of different ICL examples are sampled from the same task distribution and thus form parallel structures. \chen{I think these comparisons look defensive}\hh{I agree. This is too low level and we don't have to try hard to make them different. The reader can already see the diff from your description. (And I still don't think the diff matters.)} However, parallel structures are more flexible than ICL prompts: \textit{i)} The former specifies the relation between only \textit{two} tokens while the latter specifies the property of a long span; \textit{ii)} The former does not require the conditional distributions to be an input-output task mapping, while the latter does.

\hh{We have not stated our goal yet: why do we want to detect them?}
We first propose an algorithm to detect parallel structures in natural language (Figure~\ref{fig2}, Section~\ref{sec:detection}). \chen{Too detailed, should ground on fig 2's example} If two tokens have similar conditional distributions, fine-tuning an off-the-shelf LM on the conditional probability of the first token should also increase the conditional probability of the second token \cite{dhaliwal2018gradient, NEURIPS2019_c61f571d}. We use this intuition to score the parallel structure strength of each token pair. \hh{The last sentence is unclear: what's strength? what's a token pair (you can mention this when you define parallel structures)? It needs to be more precise without being longer, or it needs to be removed and we just leave it at the intuition level.}
% To score the parallel structure strength between any two tokens in the same document, we fine-tune an off-the-shelf LM on the first token and evaluate how much fine-tuning increases the conditional probability of the second token (the increase can be negative).

\hh{Again, why do we want to do this?}
We then study how parallel structures in the pre-training data affect the emergent ICL capability of pre-trained LMs (\mbox{Section~\ref{sec:ablation}}). We apply our algorithm to identify the parallel structures in the pre-training corpus, ablate them by injecting noise, and use the ablated corpus to continue pre-training off-the-shelf LMs.
\hh{The description is too flat. We want to emphasize that we not pretraining from scratch but instead finetune / continue pretrain a base LLM for efficiency.}
Experiments show that \textbf{ablating the parallel structures in the pre-training\hh{finetuning?} data reduces the ICL accuracy of pre-trained LMs by} $\mathbf{51.1\%}$\hh{Is this relative or absolute}, while ablating randomly sampled tokens of the same portion\hh{number?} only reduces the ICL accuracy by $1.5\%$. \chen{Readers will need more context to understand the following experiment.} 
\hh{Yes. It's unclear why long range dep and n-gram rep matter here.}
\hh{And I think the result should go in properties of PS, e.g., to compare with prior work, we categorize them into three categories and measure their influence separately.}
Parallel structures overlap with long-range dependencies and n-gram repetitions, so we conduct additional ablation experiments to distinguish their individual impacts on emergent ICL. Experiments show that \textit{i)} parallel structures are more crucial than long-range dependencies, and \textit{ii)} parallel structures that are not n-gram repetitions are also crucial.

Knowing that parallel structures are crucial for ICL to emerge, we study what they look like in natural language (Section~\ref{sec:analysis}). \chen{I think it might be more convincing to have some quantitative analysis, in addition to just examples; }
\hh{We need some story to connect these characteristics. Are they consistent or contradicting to prior results? Why did you want to measure them in the first place? What's the takeaway from these findings? For example, diversity suggests that there are many ICL tasks in pretraining, which may explain why the model generalizes to downstream tasks (connects to https://arxiv.org/abs/2306.15063)}
We find that parallel structures in natural language \textit{(i)} are common, \textit{(ii)} often span long distances, \textit{(iii)} distribute evenly, and \textit{(iv)} capture diverse semantic and syntactic patterns.
Our algorithm detects \textbf{semantic} parallel structures, ranging from n-gram repetitions (e.g., ``further improving the'' followed by ``resolution'') to simple patterns (e.g., ``\textbackslash{}n\textbackslash{}n('' followed by a year number) and more complicated patterns that require knowledge (e.g., a basketball player followed by their position).
Our algorithm also detects \textbf{syntactic} parallel structures, e.g., the same part of speech pattern (e.g., a pronoun followed by a verb), punctuation pattern, or line break pattern (Table~\ref{tab:parallel-structure-examples}). 

\hh{Can remove. The findings are already the contributions.}
Our contributions are as follows: \textit{(i)} We propose a statistical algorithm to detect parallel structures in natural language; \textit{(ii)} We show empirically with ablation experiments that parallel structures in the pre-training data are crucial for ICL to emerge; \textit{(iii)} We study the characteristics of parallel structures in natural language.

==> deprecated/ablation_results.tex <==
\begin{table*}[t]
\fontsize{11}{11}\selectfont
\setlength{\tabcolsep}{3pt}
\centering
\begin{tabular}{llcccccccccc}
\toprule
Model & Data & Tense & Adj-N & Case & Syn & Copy & LastC & Palin & Search & Pattern & Avg \\
\midrule
\multirow{7}{*}{\textsc{GPT2-S}} & \textsc{Off-the-shelf} & $29.0$ & $11.1$ & $58.8$ & $13.4$ & $21.5$ & $25.1$ & $7.7$ & $17.9$ & $33.6$ & $24.2$ \\
\cmidrule{2-12}
& \textsc{Clean} & $28.0$ & $10.4$ & $56.6$ & $12.6$ & $18.5$ & $22.9$ & $6.9$ & $16.0$ & $29.6$ & $22.4$ \\
\cmidrule{2-12}
& $-$\textsc{Random} & $18.2$ & $8.4$ & $37.5$ & $11.6$ & $9.3$ & $16.6$ & $7.1$ & $19.3$ & $27.2$ & $17.3$ \\
\cmidrule{2-12}
& $-$\textsc{Para} & $\mathbf{3.4}$ & $\mathbf{2.6}$ & $\mathbf{17.6}$ & $\mathbf{5.2}$ & $\mathbf{0.4}$ & $1.1$ & $\mathbf{-0.1}$ & $10.4$ & $\mathbf{4.9}$ & $\mathbf{5.1}$ \\
\cmidrule{2-12}
& $-$\textsc{Dep} $+$ \textsc{Para} & $8.6$ & $5.6$ & $29.3$ & $8.4$ & $2.7$ & $6.3$ & $7.9$ & $20.8$ & $20.8$ & $12.3$ \\
\cmidrule{2-12}
& $-$\textsc{Para}$+$ \textsc{Dep} & $5.7$ & $3.6$ & $21.8$ & $6.2$ & $0.4$ & $1.8$ & $0.9$ & $12.9$ & $8.9$ & $6.9$ \\
\cmidrule{2-12}
& $-$\textsc{Para}$+$ \textsc{Copy} & $3.7$ & $2.9$ & $18.4$ & $5.7$ & $0.6$ & $\mathbf{1.0}$ & $-0.1$ & $\mathbf{10.1}$ & $5.1$ & $5.3$ \\
\midrule
\multirow{7}{*}{\textsc{GPT2-M}} & \textsc{Off-the-shelf} & $54.6$ & $26.6$ & $78.4$ & $15.6$ & $30.3$ & $31.6$ & $13.1$ & $21.3$ & $39.1$ & $34.5$ \\
\cmidrule{2-12}
& \textsc{Clean} & $55.7$ & $27.2$ & $77.5$ & $17.2$ & $29.6$ & $31.9$ & $14.8$ & $22.1$ & $37.4$ & $34.8$ \\
\cmidrule{2-12}
& $-$\textsc{Random} & $55.4$ & $25.7$ & $68.0$ & $16.1$ & $24.8$ & $27.5$ & $22.9$ & $28.8$ & $45.0$ & $34.9$ \\
\cmidrule{2-12}
& $-$\textsc{Para} & $28.2$ & $\mathbf{12.0}$ & $\mathbf{52.8}$ & $9.3$ & $0.9$ & $\mathbf{4.7}$ & $\mathbf{11.3}$ & $\mathbf{17.6}$ & $14.0$ & $\mathbf{16.7}$ \\
\cmidrule{2-12}
& $-$\textsc{Dep} $+$ \textsc{Para} & $47.1$ & $22.0$ & $62.0$ & $13.5$ & $3.9$ & $15.8$ & $25.4$ & $30.0$ & $32.9$ & $28.1$ \\
\cmidrule{2-12}
& $-$\textsc{Para}$+$ \textsc{Dep} & $46.8$ & $21.8$ & $63.7$ & $13.0$ & $2.5$ & $11.7$ & $17.5$ & $24.3$ & $26.4$ & $25.3$ \\
\cmidrule{2-12}
& $-$\textsc{Para}$+$ \textsc{Copy} & $\mathbf{28.0}$ & $12.1$ & $53.3$ & $\mathbf{9.3}$ & $\mathbf{0.8}$ & $5.0$ & $11.7$ & $18.4$ & $\mathbf{13.4}$ & $16.9$ \\
\midrule
\multirow{7}{*}{\textsc{GPT2-L}} & \textsc{Off-the-shelf} & $56.1$ & $31.1$ & $83.5$ & $21.1$ & $31.8$ & $38.5$ & $10.9$ & $15.3$ & $42.4$ & $36.7$ \\
\cmidrule{2-12}
& \textsc{Clean} & $51.1$ & $33.3$ & $84.5$ & $21.2$ & $41.0$ & $38.0$ & $14.5$ & $17.5$ & $46.3$ & $38.6$ \\
\cmidrule{2-12}
& $-$\textsc{Random} & $60.4$ & $31.7$ & $75.9$ & $20.6$ & $46.6$ & $40.7$ & $23.3$ & $27.8$ & $56.5$ & $42.6$ \\
\cmidrule{2-12}
& $-$\textsc{Para} & $29.5$ & $19.6$ & $59.3$ & $12.6$ & $13.1$ & $15.9$ & $\mathbf{12.9}$ & $\mathbf{22.8}$ & $33.3$ & $24.3$ \\
\cmidrule{2-12}
& $-$\textsc{Dep} $+$ \textsc{Para} & $53.3$ & $27.8$ & $68.6$ & 
$17.3$ & $31.0$ & $31.3$ & $25.1$ & $31.5$ & $52.8$ & $37.6$ \\
\cmidrule{2-12}
& $-$\textsc{Para}$+$ \textsc{Dep} & $42.0$ & $24.4$ & $66.6$ & $14.4$ & $13.2$ & $19.9$ & $12.5$ & $22.9$ & $41.3$ & $28.6$ \\
\cmidrule{2-12}
& $-$\textsc{Para}$+$ \textsc{Copy} & $\mathbf{27.7}$ & $\mathbf{19.1}$ & $\mathbf{58.5}$ & $\mathbf{11.8}$ & $\mathbf{11.8}$ & $\mathbf{15.1}$ & $13.4$ & $23.1$ & $\mathbf{31.2}$ & $\mathbf{23.5}$ \\
\bottomrule
\end{tabular}
\caption{\label{tab:ablation} We evaluate how different ablations to the pre-training corpus affect emergent ICL capabilities of LMs. Parallel structures are crucial for ICL to emerge. LMs further pre-trained on data with \underline{parallel structures ablated} consistently underperform LMs further pre-trained on data with \underline{random tokens ablated} on all nine evaluation tasks and all three model sizes, by $\mathbf{70.7\%}$ on \mbox{GPT2-Small}, $\mathbf{52.0\%}$ on GPT2-Medium, and $\mathbf{42.9\%}$ on GPT2-Large (relative). See Section~\ref{sec:ablation-results} for additional analysis.}
\end{table*}

==> deprecated/parallel_structure_examples.tex <==
\begin{table*}[t]
\small
\begin{tabular}{p{0.45in} p{1.0in} p{1.4in} p{1.4in} p{1in}}
\toprule
\multicolumn{2}{l}{Pattern Type} & Text 1 & Text 2 & Pattern\\
\midrule
Semantic & ngram & Gun Safety Action Fund (New York): \textbf{2014 — \$} & ot Group (Las Vegas): \textbf{2014 — \$} & "2014 — \$" \\
\cmidrule{2-5}
& ngram variants (synonyms / antonyms) & compared to other twin strollers. You \textbf{can} & ches. It’s fast and easy, a \textbf{useful} & synonyms \\
\cmidrule{3-5}
&  & didn’t prevent Rome’s \textbf{decline and fall} & fur traders. Most American cities \textbf{arose} & antonyms \\
\cmidrule{2-5}
& topic & before Prestatyn Magistrates' \textbf{Court charged} & Evans was seeking the leave of the \textbf{Court of Appeal} to \textbf{appeal} & legal court \\
\cmidrule{3-5}
&  & from his post-hardcore supergroup \textbf{Sianvar} & am—guitar insanity. But for \textbf{Stay Lost} & music\\
\cmidrule{2-5}
& dimension (quantity / location / time) & ongs'\textbackslash{}n\textbackslash{}nAn \textbf{initial} meeting between the two sparked & excited about the music.\textbackslash{}n\textbackslash{}nIn \textbf{2007} & time \\
\cmidrule{3-5}
&  & seminations) was approximately \textbf{14 times} & (\textbf{n = 17} eggs in each group, \textbf{mean proportion} & quantity\\
\cmidrule{2-5}
& language & ună cu planeta de m & ieții, aș & Romanian \\
\cmidrule{3-5}
&  & de registrar tu música sin t & el trastero, te harán plante & Spanish \\
\cmidrule{3-5}
&  & ://www.lewismoten. & ://thecontroversialfiles.com & Web Link \\
\midrule
Syntactic & part-of-speech & associated with Christendom arrangements.\textbackslash{}n\textbackslash{}n\textbf{It is} & may be the case, but that is the way \textbf{I have} & Pronoun $\rightarrow$ Verb \\
\cmidrule{3-5}
&  & endogenous decision--banks could always \textbf{choose to} & stable funding model and their \textbf{investing in} & Verb $\rightarrow$ Preposition \\
\cmidrule{2-5}
& punctuation & OL apparently awarded the contracts to \textbf{U.}' & FOCUS ON TRAININ\textbf{G,} & Capitalized word $\rightarrow$ Punctuation \\
\cmidrule{2-5}
& break & Powder \textbf{141\textbackslash{}n}, & Oil and Water, Experiments with \textbf{161\textbackslash{}n} & Number $\rightarrow$ \textbackslash{}n \\
\bottomrule
\end{tabular}
\caption{\label{tab:parallel-structure-examples} Our algorithm detects diverse parallel structures covering different semantic and syntactic patterns. The bolded tokens are the parallel structures that share the same pattern.
}
\end{table*}


==> tables/parallel_structure_examples.tex <==
\begin{table*}[t]
\centering
\fontsize{9}{9}\selectfont
\begin{tabular}{p{0.5in} p{1.6in} p{1.6in} p{1.6in}}
\toprule
 & Former Context \& Token & Latter Context \& Token & Shared Distribution\\ 
\midrule
Semantics & be added by further improving the \textbf{resolution} & maps (“By further improving the \textbf{resolution} & same ngram (further improving the $\Rightarrow$ resolution) \\ 
\cmidrule{2-4}
 & ", you have to either cd to the parent \textbf{directory} & the remote-machine and places it in \textbf{\textasciitilde{}/.} & preposition $\Rightarrow$ synonyms (to/in $\Rightarrow$ the parent directory or \textasciitilde{}/.) \\ 
\cmidrule{2-4}
 & Gambia Georgia Germany Ghana Greece Grenada Guam Guatemala \textbf{Guantanamo} & Senegal Serbia Seychelles Sierra Leone Singapore Slovakia Slovenia \textbf{Somalia} & location names ordered by alphabetic order \\ 
\cmidrule{2-4}
 & st du doch niemals wer\textbf{den} & uf und will, dass man i\textbf{hr} & German language \\ 
\cmidrule{2-4}
 & \textbackslash{}n- -\textbackslash{}n\textbackslash{}n\textbf{1974} & ones I mean.\textbackslash{}n\textbackslash{}n- -\textbackslash{}n\textbackslash{}n\textbf{2010} & \textbackslash{}n\textbackslash{}n $\Rightarrow$ a year \\ 
\cmidrule{2-4}
 & Ed Morrow, \textbf{PF} & So, Bryce Peters, \textbf{SG} & basketball player $\Rightarrow$ their position \\ 
\midrule
Syntax & “Well… you’\textbf{re} & once more. “I’\textbf{m} & part of speech pattern (pronoun $\Rightarrow$ verb) \\ 
\cmidrule{2-4}
& sites near or on the ground\textbf{.[} & brate predation occurred when larvae were in the litter\textbf{.[} & punctuation pattern (prepositional phrases $\Rightarrow$ .[) \\
\cmidrule{2-4}
& \textbackslash{}n\textbackslash{}nEND\textbackslash{}n\textbackslash{}nEND Preorder;\textbf{\textbackslash{}n\textbackslash{}n} & INC ( i )\textbackslash{}n\textbackslash{}nEND ;\textbf{\textbackslash{}n\textbackslash{}n} & line break pattern (; $\Rightarrow$ \textbackslash{}n\textbackslash{}n) \\ 
\bottomrule
\end{tabular}
\caption{\label{tab:parallel-structure-examples} Our algorithm detects parallel structures with diverse semantic and syntactic patterns. The two tokens that form parallel structures are \textbf{bold}. $\Rightarrow$ denotes ``followed by''.
}
\end{table*}
